Efficient and Explicit Modelling of Image Hierarchies for Image Restoration

The aim of this paper is to propose a mechanism to efficiently and explicitly model image hierarchies in the global, regional, and local range for image restoration. To achieve that, we start by analyzing two important properties of natural images including cross-scale similarity and anisotropic image features. Inspired by that, we propose the anchored stripe self-attention which achieves a good balance between the space and time complexity of self-attention and the modelling capacity beyond the regional range. Then we propose a new network architecture dubbed GRL to explicitly model image hierarchies in the Global, Regional, and Local range via anchored stripe self-attention, window self-attention, and channel attention enhanced convolution. Finally, the proposed network is applied to 7 image restoration types, covering both real and synthetic settings. The proposed method sets the new state-of-the-art for several of those. Code will be available at https://github.com/ofsoundof/GRL-Image-Restoration.git.

==> figures/visual_dn.tex <==
\begin{figure*}[!tb]
\begin{center}
\scriptsize
% \scalebox{0.97}{
\begin{tabular}[b]{c@{ } c@{ } c@{ } c@{ }}
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_gt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_noisy.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_sgn.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_drunet.png} \\
    Ground-truth & Noisy & SGN~\cite{gu2019self} & DRUNet~\cite{zhang2021plug}  \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_ipt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_swinir.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_003_grl.png} \\ 
    IPT~\cite{chen2021pre} & SwinIR~\cite{liang2021swinir} & Restormer~\cite{zamir2022restormer} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_gt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_noisy.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_sgn.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_drunet.png} \\
    Ground-truth & Noisy & SGN~\cite{gu2019self} & DRUNet~\cite{zhang2021plug}  \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_ipt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_swinir.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_004_grl.png} \\ 
    IPT~\cite{chen2021pre} & SwinIR~\cite{liang2021swinir} & Restormer~\cite{zamir2022restormer} & GRL  \\ \\
% \hspace{-2mm}  
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_gt.png} &
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_noisy.png} & 
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_sgn.png} &
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_drunet.png} \\
    % Ground-truth & Noisy & SGN~\cite{gu2019self} & DRUNet~\cite{zhang2021plug}  \\
% \hspace{-2mm}  
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_ipt.png} &
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_swinir.png} & 
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_restormer.png} &
%     \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_005_grl.png} \\ 
    % IPT~\cite{chen2021pre} & SwinIR~\cite{liang2021swinir} & Restormer~\cite{zamir2022restormer} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_gt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_noisy.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_sgn.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_drunet.png} \\
    Ground-truth & Noisy & SGN~\cite{gu2019self} & DRUNet~\cite{zhang2021plug}  \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_ipt.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_swinir.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dn50/img_012_grl.png} \\ 
    IPT~\cite{chen2021pre} & SwinIR~\cite{liang2021swinir} & Restormer~\cite{zamir2022restormer} & GRL  \\ \\
\end{tabular}
% }
\end{center}
% \vspace{-4mm}
\caption{Visual results for color image denoising. The noise level is 50. Compared with the other methods, the proposed method could restore more details in the input image while removing severe noise from the input images.}
% Instead, the combination of the horizontal and vertical stripes and their shifted version could be well suited to the anisotropic features. Conducting self-attention could further reduce the computational complexity and maintain the long-range modelling capacity.}
\label{fig:supp_visual_dn}
% \vspace{-6mm}
\end{figure*}


==> figures/visual_dpdd.tex <==
\begin{figure*}[!tb]
\begin{center}
\scriptsize
% \scalebox{0.97}{
\begin{tabular}[b]{c@{ } c@{ } c@{ } c@{ }}
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2316_lq.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2316_uformer.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2316_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2316_grl.png} \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A0995_lq.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A0995_uformer.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A0995_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A0995_grl.png} \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A1652_lq.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A1652_uformer.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A1652_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A1652_grl.png} \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2002_lq.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2002_uformer.png} & 
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2002_restormer.png} &
    \includegraphics[width=0.24\linewidth,valign=t]{latex/images_supp/dpdd/1P0A2002_grl.png} \\ \\

    Blurred & Uformer~\cite{wang2022uformer} & Restormer~\cite{zamir2022restormer} & GRL  \\
\end{tabular}
% }
\end{center}
% \vspace{-4mm}
\caption{Visual results for dual-pixel defocus deblurring. Compared with other methods, the proposed method could remove more blurriness from the input image.}
% Instead, the combination of the horizontal and vertical stripes and their shifted version could be well suited to the anisotropic features. Conducting self-attention could further reduce the computational complexity and maintain the long-range modelling capacity.}
\label{fig:supp_visual_dpdd}
% \vspace{-6mm}
\end{figure*}


==> figures/visual_motion_db.tex <==
\begin{figure*}[!tb]
\begin{center}
\scriptsize
% \scalebox{0.97}{
\begin{tabular}[b]{c@{ } c@{ } c@{ } c@{ } c@{ }}
\hspace{-2mm}  
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_lq.png} &
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_mprnet.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_uformer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_restormer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0410_11_00_00000069_grl.png}  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_lq.png} &
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_mprnet.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_uformer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_restormer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0854_11_00_00000089_grl.png}  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_lq.png} &
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_mprnet.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_uformer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_restormer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0862_11_00_00000043_grl.png}  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_lq.png} &
    \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_mprnet.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_uformer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_restormer.png} & \includegraphics[width=0.19\linewidth,valign=t]{latex/images_supp/motion_db/GOPR0881_11_01_00000012_grl.png}  \\ \\
    Blurred & MPRNet~\cite{zamir2021multi} & Uformer~\cite{wang2022uformer} & Restormer~\cite{zamir2022restormer} & GRL (Ours) \\
\end{tabular}
% }
\end{center}
% \vspace{-4mm}
\caption{Visual results for single image motion deblurring. The proposed method GRL could recover sharper details compared with the other methods.}
% Instead, the combination of the horizontal and vertical stripes and their shifted version could be well suited to the anisotropic features. Conducting self-attention could further reduce the computational complexity and maintain the long-range modelling capacity.}
\label{fig:supp_visual_motion_db}
% \vspace{-6mm}
\end{figure*}

==> figures/visual_sr.tex <==
\begin{figure*}[!tb]
\begin{center}
\scriptsize
% \scalebox{0.97}{
\begin{tabular}[b]{c@{ } c@{ } c@{ }}
% \hspace{-2mm}  
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_gt.png} &
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_lr.png} & 
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_ipt.png} \\
%     Ground-truth & LR & IPT~\cite{chen2021pre}  \\
% \hspace{-2mm}  
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_swinir.png} &
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_edt.png} &
%     \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_003_grl.png} \\ 
    % SwinIR~\cite{liang2021swinir} & EDT~\cite{li2021efficient} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_gt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_lr.png} & 
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_ipt.png} \\
    Ground-truth & LR & IPT~\cite{chen2021pre}  \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_swinir.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_edt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_019_grl.png} \\ 
    SwinIR~\cite{liang2021swinir} & EDT~\cite{li2021efficient} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_gt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_lr.png} & 
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_ipt.png} \\
    Ground-truth & LR & IPT~\cite{chen2021pre}  \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_swinir.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_edt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_020_grl.png} \\ 
    SwinIR~\cite{liang2021swinir} & EDT~\cite{li2021efficient} & GRL  \\ \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_gt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_lr.png} & 
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_ipt.png} \\
    Ground-truth & LR & IPT~\cite{chen2021pre}  \\
\hspace{-2mm}  
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_swinir.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_edt.png} &
    \includegraphics[width=0.25\linewidth,valign=t]{latex/images_supp/srx4/img_024_grl.png} \\ 
    SwinIR~\cite{liang2021swinir} & EDT~\cite{li2021efficient} & GRL  \\ \\

\end{tabular}
% }
\end{center}
\vspace{-4mm}
\caption{Visual results for classical image SR. The upscaling factor is $\times 4$. Compared with other methods, the proposed method could recover more details such as lines and edges in the input LR image.}
% Instead, the combination of the horizontal and vertical stripes and their shifted version could be well suited to the anisotropic features. Conducting self-attention could further reduce the computational complexity and maintain the long-range modelling capacity.}
\label{fig:supp_visual_sr}
% \vspace{-6mm}
\end{figure*}
